InstaFlow: One Step is Enough for High-Quality Diffusion-Based Text-to-Image Generation

Diffusion models have revolutionized text-to-image generation with its exceptional quality and creativity. However, its multi-step sampling process is known to be slow, often requiring tens of inference steps to obtain satisfactory results. Previous attempts to improve its sampling speed and reduce computational costs through distillation have been unsuccessful in achieving a functional one-step model. In this paper, we explore a recent method called Rectified Flow, which, thus far, has only been applied to small datasets. The core of Rectified Flow lies in its \emph{reflow} procedure, which straightens the trajectories of probability flows, refines the coupling between noises and images, and facilitates the distillation process with student models. We propose a novel text-conditioned pipeline to turn Stable Diffusion (SD) into an ultra-fast one-step model, in which we find reflow plays a critical role in improving the assignment between noise and images. Leveraging our new pipeline, we create, to the best of our knowledge, the first one-step diffusion-based text-to-image generator with SD-level image quality, achieving an FID (Frechet Inception Distance) of $23.3$ on MS COCO 2017-5k, surpassing the previous state-of-the-art technique, progressive distillation, by a significant margin ($37.2$ $\rightarrow$ $23.3$ in FID). By utilizing an expanded network with 1.7B parameters, we further improve the FID to $22.4$. We call our one-step models \emph{InstaFlow}. On MS COCO 2014-30k, InstaFlow yields an FID of $13.1$ in just $0.09$ second, the best in $\leq 0.1$ second regime, outperforming the recent StyleGAN-T ($13.9$ in $0.1$ second). Notably, the training of InstaFlow only costs 199 A100 GPU days. Codes and pre-trained models are available at \url{github.com/gnobitab/InstaFlow}.

==> tex/conclusion.tex <==
\section{The Best is Yet to Come}
The recurrent nature of diffusion models hinders their deployment on edge devices~\cite{li2023snapfusion, stable-diffusion-coreml-apple-silicon}, harms user experience, and adds to the overall cost. In this paper, we demonstrate that a powerful one-step generative model can be obtained from pre-trained Stable Diffusion (SD) using the text-conditioned Rectified Flow framework. Based on our results, we propose several promising future directions for exploration:

\begin{enumerate}
    \item \textbf{Improving One-Step SD}: The training of the 2-Rectified Flow model did not fully converge, despite investing 75.2 A100 GPU days.
    This is only a fraction of training cost of the original SD ($6250$ A100 GPU days). By scaling up the dataset, model size, and training duration, we believe the performance of one-step SD will improve significantly. Moreover, SOTA base models, e.g., SDXL~\cite{podell2023sdxl}, can be leveraged as teachers to enhance the one-step SD model.
    
    \item \textbf{One-Step ControlNet~\cite{zhang2023adding}}: By applying our pipeline to train ControlNet models, it is possible to get one-step ControlNets capable of generating controllable contents within milliseconds. The only required modification involves adjusting the model structure and incorporating the control modalities as additional conditions.

    \item \textbf{Personalization for One-Step Models}: By fine-tuning SD with the training objective of diffusion models and LORA~\cite{hu2021lora} , users can customize the pre-trained SD to generate specific contents and styles~\cite{ruiz2023dreambooth}. However, as the one-step models have substantial difference from traditional diffusion models, determining the objective for fine-tuning these one-step models remains a subject that requires further investigation.    

    \item \textbf{Neural Network Structure for One-Step Generation}: It is widely acknowledged in the research community that the U-Net structure plays a crucial role \cite{songscore, ho2020denoising, dhariwal2021diffusion} in the impressive performance of diffusion models in image generation. With the advancement of creating one-step SD models using text-conditioned reflow and distillation, several intriguing directions arise: (1) exploring alternative one-step structures, such as successful architectures~\cite{sauer2023stylegan, kang2023scaling, karras2019style, karras2020analyzing} used in GANs, that could potentially surpass the U-Net in terms of quality and efficiency; (2) leveraging techniques like pruning, quantization, and other approaches for building efficient neural networks to make one-step generation more computationally affordable while minimizing potential degradation in quality.

\end{enumerate}

